Learning with Imperfect Models: When Multi-step Prediction Mitigates Compounding Error

Compounding error, where small prediction mistakes accumulate over time, presents a major challenge in learning-based control. For example, this issue often limits the performance of model-based reinforcement learning and imitation learning. One common approach to mitigate compounding error is to train multi-step predictors directly, rather than relying on autoregressive rollout of a single-step model. However, it is not well understood when the benefits of multi-step prediction outweigh the added complexity of learning a more complicated model. In this work, we provide a rigorous analysis of this trade-off in the context of linear dynamical systems. We show that when the model class is well-specified and accurately captures the system dynamics, single-step models achieve lower asymptotic prediction error. On the other hand, when the model class is misspecified due to partial observability, direct multi-step predictors can significantly reduce bias and thus outperform single-step approaches. These theoretical results are supported by numerical experiments, wherein we also (a) empirically evaluate an intermediate strategy which trains a single-step model using a multi-step loss and (b) evaluate performance of single step and multi-step predictors in a closed loop control setting.

==> tex/brainstorming.tex <==
\subsection{Related Work}

- Model fitting. 
- Finite sample analysis (transient effects, different burn-in times)
\begin{itemize}
    \item \url{https://arxiv.org/pdf/2002.04523}
    \item \url{https://arxiv.org/pdf/2012.09156}
    \item \url{https://arxiv.org/pdf/2203.09637}
    \item \url{https://arxiv.org/abs/2409.10405} and references therein
    \item \url{https://arxiv.org/pdf/2301.04104} World models
    \item \url{https://arxiv.org/pdf/1704.02254}
\end{itemize}

Can characterize prediction error in terms of system quantities. Can then minimize prediction error as a function of the planning horizon. 

Include misspecification and  multi-step roll out error. \\
- Expand things out \\ 
- Give a few linear examples and interpretation. \\ 
- Give a few nonlinear examples and interpretation ... cartpole (fully observed, partially observed) \\
With well-specified models, it is asymptotically best to do single step prediction \\
With misspecification, it may depends highly on the system and the nature of misspecification \\
-Take unicycle model, and try to fit linear dynamics. \\ 

- For numerical comparisons, include -prediction error, MPC control error with fixed parameters. Compare these for single step models with single and multi-step costs, as well as multi-step models. 

-Sit down with Anne to write the general results. Highlight the special cases to fill in and numerical experiments to run with them. 

\section{General Formulation}

Consider the POMDP described by
\begin{align*}
    Y_{t+1  } \sim p(Y_{t+1} \vert Y_{-\infty:t}, U_{-\infty:t})
\end{align*}
for some unknown density $p$. A model for the data generating process may be formed by performing density estimation by forming a predictive model
for a collection of indices $t+1:t+k$: \begin{align*}
    \hat Y_{t+1:t+k} \sim \hat f(Y_{t+1:t+k} \vert Y_{-\infty:t}, U_{-\infty:t}, \theta_U)
\end{align*}
for some $k > 0$. A typical approach for selecting is to set the loss function as the negative logarithm of the density $f \in \calF$ for some hypothesis class $\calF$. The optimization problem then becomes 
\begin{align*}
    \hat f = \argmin_{f \in \calF} - \sum_{(Y_{t+1: t+k}, Y_{-\infty:t}, U_{-\infty:t}) \in \calD} \log f(Y_{t+1:t+k} | Y_{-\infty:t}, U_{-\infty:t}, \theta_U). 
\end{align*}

This formulation captures
\begin{itemize}
    \item Single step prediction error minimization by taking $k = 1$. Then the above objective becomes the (pseudo-)maximum likelihood objective\footnote{It is referred to as pseudo-maximum likelihood when $p \notin \calF$.}. 
    \item Operator learning/simulation error minimization by taking $k > 1$ and letting $\calF$ consist consist of models which directly predict $1-k$ steps ahead.
    \item Single step stationary models with multi-step loss by taking $k > 1$ and letting each $f \in \calF$ be determined as the composition of single step models  $f' \in \calF'$. 
\end{itemize}

Regardless of which formulation we choose, we typically require the model to make multi-step predictions for simulaion and control purposes. In this work, we theoretically and empirically study the multi-step prediction performance of the above approaches. In particular, we theoretically compare 1 and 2 when the underlying data generating process is a linear dynamical system, and the model class is a finite impulse response model. We empirically compare $1$, $2$ and $3$ for simulations of linear and nonlinear systems. Our results lead to the following conclusions:
\begin{itemize}
    \item Single step prediction is preferred if the model is well-specified 
    \item If the model is not well-specified, there are situations where multi-step prediction is provably preferred, evidenced by finite sample bounds. These situations and the ideal prediciton horizon depend heavily upon the stability of the system and the nature of the model classes. 
    \item Minimizing the multi-step loss is often outperforms the other two methods empirically. However, this is at the cost of solving a more complex optimization problem. 
\end{itemize}

The theoretical comparison results are already sufficiently complete. We just need to back them up with numerical evidence. Let's try to draft the theoretical results into the section of our CDC paper in the next week. Talk through how to draft those results. 

Experiments: 
- Linear systems -- nearly complete. 
- Cartpole --  Neural network predictions. Vary the size of the neural network. Vary the observation protocol. Try all three approaches. Ask Anne to meet twice per week for two hours to prepare the paper for CDC. 

\section{Introduction}


Consider a linear dynamical system evolving according to 
\begin{equation}
\begin{aligned}
    \label{eq: linsys}
    X_{t+1} &= A X_t + W_t \\
    Y_t &= C X_t + V_t,
\end{aligned}
\end{equation}
for $t \geq 0$, where $X_t \in \R^{\dx}$ is the system state, $W_t \in \R^{\dx}$ is the process noise, $Y_t \in \R^{\dy}$ is the observation, and $V_t \in \R^{\dy}$ is measurement noise.  The matrices $A \in \R^{\dx \times \dx}$ and $C \in \R^{\dy \times\dx}$ are unknown. 

A common approach to design such models has been to 
1. fit an autoregressive model for one step ahead prediction
2. roll this prediction out by evaluating the prediction, and feeding this back into the model. 

However, perhaps unsurprisingly, optimizing a one-step objective, and attempting to use this to make predictions in the fashion above may be suboptimal. Indeed, it is found in model-based reinforcement learning that .... Similarly, language models are often trained on 

The objective in the forecasting problem is to use the measurements up to time $t$ to predict the measurements at time $t+1, \dots t+n$. Denote such a predictor as $\hat y_{t+1:t+N|t} = G(y_{0:t})$. The optimal such predictor takes the form of a Kalman Filter:
\begin{align*}
    \hat x_{t+1} &= A \hat x_t + K y_t \\
    y_t &= C \hat x_t. 
\end{align*}
The forecasting objective is given by 
\begin{align*}
    \calC(G) = \mathbf{E}\brac{\sum_{t=0}^T \norm{y_{t+1:t+N} - G(y_{0:t})}^2}. 
\end{align*}
\Bruce{Include some matrix multiplying $y_t$ in the objectve for defining the forecasting objective. }

\Bruce{Use the definition of this objective to decompose the cost into the unavoidable component and the estimation error. }

\Bruce{We consider a learner who interacts with the system \eqref{eq: linsys} to }

Direct trajectory prediction offers many potential benefits over autoregressive evaluation. However, it is clearly not always dominant, and ... 

In this work, we characterize situations. 

Our analysis from such simple, analytically tractable settings is backed up by experiments with ...

We perform evaluation on simple benchmark tasks. Our evaluations demonstrate that in situations where 
\begin{enumerate}
    \item Linear systems
    \item Simulated nonlinear systems: Consider a cartpole system. Known parametric form... Can set 
    \item Consider 
\end{enumerate}

Focus on trajectory prediction, apply MBRL in this setting. 

Try out this more classical approach in comparison to 

==> tex/discussion.tex <==
\section{Discussion}


